The First AI4TSP Competition: Learning to Solve Stochastic Routing Problems

This paper reports on the first international competition on AI for the traveling salesman problem (TSP) at the International Joint Conference on Artificial Intelligence 2021 (IJCAI-21). The TSP is one of the classical combinatorial optimization problems, with many variants inspired by real-world applications. This first competition asked the participants to develop algorithms to solve a time-dependent orienteering problem with stochastic weights and time windows (TD-OPSWTW). It focused on two types of learning approaches: surrogate-based optimization and deep reinforcement learning. In this paper, we describe the problem, the setup of the competition, the winning methods, and give an overview of the results. The winning methods described in this work have advanced the state-of-the-art in using AI for stochastic routing problems. Overall, by organizing this competition we have introduced routing problems as an interesting problem setting for AI researchers. The simulator of the problem has been made open-source and can be used by other researchers as a benchmark for new AI methods.

==> result_tables.tex <==
% \documentclass[preprint, 3p, 11pt, authoryear]{elsarticle}
% %\documentclass{elsarticle}
% \usepackage{lineno,hyperref}
% \usepackage{times}
% \usepackage{soul}
% \usepackage{url}
% \usepackage[utf8]{inputenc}
% \usepackage[small]{caption}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{booktabs}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{dsfont}
% \usepackage{amsmath}
% %\usepackage[caption=false]{subfig}
% % \usepackage{caption}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \sloppy
% % \urlstyle{same}
% \usepackage{subcaption}


% \modulolinenumbers[5]

% %
% \journal{Artificial Intelligence}

% %%%%%%%%%%%%%%%%%%%%%%%
% %% Elsevier bibliography styles
% %%%%%%%%%%%%%%%%%%%%%%%
% %% To change the style, put a % in front of the second line of the current style and
% %% remove the % from the second line of the style you would like to use.
% %%%%%%%%%%%%%%%%%%%%%%%

% %% Numbered
% \bibliographystyle{model1-num-names}

% %% Numbered without titles
% %\bibliographystyle{model1a-num-names}

% %% Harvard
% %\bibliographystyle{model2-names.bst}\biboptions{authoryear}

% %% Vancouver numbered
% %\usepackage{numcompress}\bibliographystyle{model3-num-names}

% %% Vancouver name/year
% %\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

% %% APA style
% %\bibliographystyle{model5-names}\biboptions{authoryear}

% %% AMA style
% %\usepackage{numcompress}\bibliographystyle{model6-num-names}

% %% `Elsevier LaTeX' style
% % \bibliographystyle{elsarticle-num}
% %%%%%%%%%%%%%%%%%%%%%%%

% \begin{document}

% \begin{table}[tbp]
% % \begin{minipage}[c]{0.1\textwidth}
%     \centering
%     %\caption{Leaderboard for the validation phase.}
%     %\label{tab:leaderboard_val}
%     \begin{subtable}[c]{0.5\textwidth}
%     \subcaption{Leaderboard for the validation phase.}
%     \label{tab:leaderboard_val}
%     \begin{tabular}{c|c}
%     \toprule
%         \multicolumn{2}{c}{Track 1}\\
%         \midrule
%          ZLI & 8.404499999999793  \\
%          Convexers & 7.8099999999988885\\
%          Margaridinhas & 7.533834999999982
%          \\
%          Topline & 3.540000000000663\\
%          VK & 0.5300000000000102\\
%          \midrule
%          \multicolumn{2}{c}{Track 2}\\
%          \midrule
%          Ratel & 10.69104\\
%          ML for TSP & 9.82955\\
%          RISEup & 9.16567\\
%          VK & -6.69772\\
%          UniBw & -13.14861\\
%     \bottomrule
%     \end{tabular}
%     \captionof{table}{Leaderboard for the validation phase.}%\label{tab:leaderboard_val}
% % \end{minipage}%
% \end{subtable}
% %\end{table}
% % \begin{minipage}[c]{0.2\textwidth}
% %\begin{table}[tbp]
%     % \centering
%     % \caption{Leaderboard for the final test phase.}
%     % \label{tab:leaderboard_final}
%     \begin{subtable}[c]{0.5\textwidth}
%     \begin{tabular}{c|c}
%     \toprule
%         \multicolumn{2}{c}{Track 1}\\
%         \midrule
%          ZLI & 11.320000000002786  \\
%          Margaridinhas & 11.320000000002786
%          \\
%          Convexers & 11.320000000002786
%          \\
%          Topline & 4.300000000000301\\
%          \midrule
%          \multicolumn{2}{c}{Track 2}\\
%          \midrule
%          RISEup & 10.77341\\
%          Ratel & 10.58859\\
%          ML for TSP & 10.39341\\
%     \bottomrule
%     \end{tabular}
%     \captionof{table}Leaderboard for the final test phase.}%\label{tab:leaderboard_final}
% \end{subtable}
% % \end{minipage}
% \end{table}


\begin{table}[tbp]
    \caption{Leaderboard for the validation phase and the final test phase at deadline.}
    \label{tab:results}
    \centering
    \begin{tabular}{cc|cc}
    %\multicolumn{2}{c}{Validation phase} & \multicolumn{2}{c}{Test phase}\\
    \toprule
        Track 1 & Validation phase & Track 1 & Test phase\\%\multicolumn{4}{c}{Track 1}\\
        \midrule
         ZLI & 8.404499999999793 & ZLI & 11.320000000002786  \\
         Convexers & 7.8099999999988885 & Margaridinhas & 11.320000000002786\\
         Margaridinhas & 7.533834999999982 & Convexers & 11.320000000002786
         \\
         Topline & 3.540000000000663 & Topline & 4.300000000000301\\
         VK & 0.5300000000000102\\
         \midrule
         %\multicolumn{4}{c}{Track 2}\\
         Track 2 & Validation phase & Track 2 & Test phase\\
         \midrule
         Ratel & 10.69104 & RISEup & 10.77341\\
         ML for TSP & 9.82955 & Ratel & 10.58859\\
         RISEup & 9.16567 & ML for TSP & 10.39341\\
         VK & -6.69772 & & \\
         UniBw & -13.14861 & & \\
    \bottomrule
    \end{tabular}
    
\end{table}

\end{document}
